Estimating Risk-Aware Flexibility Areas for EV Charging Pools via Stochastic AC-OPF

This paper introduces a stochastic AC-OPF (SOPF) for the flexibility management of electric vehicle (EV) charging pools in distribution networks under uncertainty. The SOPF considers discrete utility functions from charging pools as a compensation mechanism for eventual energy not served to their charging tasks. An application of the proposed SOPF is described where a distribution system operator (DSO) requires flexibility to each charging pool in a day-ahead time frame, minimizing the cost for flexibility while guaranteeing technical limits. Flexibility areas are defined for each charging pool and calculated as a function of a risk parameter involving the solution's uncertainty. Results show that all players can benefit from this approach, i.e., the DSO obtains a risk-aware solution, while charging pools/tasks perceive a reduction in the total energy payment due to flexibility services.

==> Notation.tex <==
\vspace{-5pt}
\noindent \emph{Sets}
\begin{description}[itemsep=0.2ex, labelwidth=1.2cm, leftmargin=1.4cm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \item[$\Omega_{b}$] Set of nodes
\item[$\Omega_{f}$] Set of phases \{A, B, C\}
\item[$\Omega_{g}$] Set of nodes with distributed generation (DG) units
\item[$\Omega_{l}$] Set of distribution lines
\end{description}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \emph{Parameters}
\begin{description}[itemsep=0.2ex, labelwidth=1.2cm, leftmargin=1.4cm]
\item[\normalfont$\rm{c}$$_g^{\rm{DG}}$] Unitary generation cost at DG unit $g$ [\$/kW]
\item[\normalfont$\rm{c}^{\rm{ES}}$] Unitary generation cost at the substation [\$/kW]
\item[\normalfont$\overline{\rm{I}}_{kj}$] Maximum current magnitude at line $kj$ [A]
\item[$\rm{P}$$_{k,f}^{\rm{D}}$] Active power demand at node $k$, phase $f$ [kW]
\item[$\overline{\rm{P}}$$_{g}$] Maximum active power by generator at bus $g$ [kW]
\item[$\underline{\rm{P}}$$_{g}$] Minimum active power by generator at bus $g$ [kW]
\item[\normalfont$\rm{pf}$$_{g}$] Minimum power factor at DG unit $g$.
\item[\normalfont$\rm{Q}$$_{k,f}^{\rm{D}}$\rule{0pt}{2.3ex}] Reactive power demand at node $k$, phase $f$ [kVAr]
\itemsep=0.20ex\item[\normalfont$\rm{R}$$_{kj,f,f'}$] Resistance of line $kj$ between phases $f$ and $f'$ [$\Omega$]
\item[\normalfont$\overline{\rm{V}}$\rule{0pt}{2.3ex}] Maximum voltage magnitude [pu]
\item[\normalfont$\underline{\rm{V}}$] Minimum voltage magnitude [pu]
\item[$\rm{X}$$_{kj,f,f'}] Reactance of line $kj$ between phases $f$ and $f'$ [$\Omega$]
\item[$\Theta$] Defined angle range [$^\circ$]
\end{description}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \emph{Variables}
\begin{description}[itemsep=0.2ex, labelwidth=1.2cm, leftmargin=1.4cm]
\item[$i^{\rm{r}}_{kj,f}$  $i^{\rm{i}}_{kj,f}$] Real and imaginary parts of the current at line $kj$, phase $f$ [A]
\item[$i^{\rm{r\,D}}_{k,f}$  $i^{\rm{i\,D}}_{k,f}$] Real and imaginary parts of the load current at node $k$, phase $f$ [A]
\item[$i^{\rm{r\,DG}}_{g,f}$  $i^{\rm{i\,DG}}_{g,f}$] Real and imaginary parts of the current at DG unit $g$, phase $f$ [A]
\item[$i^{\rm{r\,ES}}_{k,f}$  $i^{\rm{i\,ES}}_{k,f}$] Real and imaginary parts of the current at the substation bus $k$, phase $f$ [A]
\item[$P^{\rm{ES}}$$]  Active power injection at the substation [kW]
\item[{$P^{\rm{DG}}_{g}$ $Q^{\rm{DG}}_{g}$}]  Active and reactive power generations at DG unit $g$ [kW, kvar]
\item[$v^{\rm{r}}_{k,f}$  $v^{\rm{i}}_{k,f}$] Real and imaginary parts of the voltage at node $k$, phase $f$ [V] 
\item[$\mu_g$] Unit status of DG unit at bus $g$ 
\end{description}


